Human Motion Capture Using a Drone

Current motion capture (MoCap) systems generally require markers and multiple calibrated cameras, which can be used only in constrained environments. In this work we introduce a drone-based system for 3D human MoCap. The system only needs an autonomously flying drone with an on-board RGB camera and is usable in various indoor and outdoor environments. A reconstruction algorithm is developed to recover full-body motion from the video recorded by the drone. We argue that, besides the capability of tracking a moving subject, a flying drone also provides fast varying viewpoints, which is beneficial for motion reconstruction. We evaluate the accuracy of the proposed system using our new DroCap dataset and also demonstrate its applicability for MoCap in the wild using a consumer drone.

==> abstract.tex <==
%!TEX root = main.tex

We present a novel system for 3D human motion capture (MoCap) by leveraging the mobility of an autonomously flying drone. Compared to traditional MoCap systems, the proposed system doesn't require markers or multiple calibrated cameras and is applicable either indoors or outdoors. Besides the capability of tracking a subject, the mobility of a flying drone also provides sufficiently fast viewpoint change during video recording, which is important for reconstructing a dynamic structure from a video. We also take advantage of the recent advances in 2D and 3D human pose estimation to obtain reliable 2D tracks of body joints and robust initialization for 3D pose reconstruction.  In addition, we propose a novel rank-1 constraint to model the articulation of human body. We validate the proposed approach using a standard benchmark for general pose estimation (Human3.6M) and a newly-collected dataset for drone-based human motion capture (DroCap), on both of which we achieve robust and accurate reconstruction without model training for the specific datasets. We also demonstrate that the proposed reconstruction pipeline is readily applicable to a consumer drone for motion capture in the wild. 

==> motivation.tex <==
Capturing the 3D full-body human pose is a challenging problem with many applications. When humans wear markers, the problem has been solved with multiple cameras in motion capture (MoCap) systems. However, the MoCap system suffers from its inflexibility -- the cameras require fixation and calibration and the subject should wear markers and be restricted within in the field of views of cameras. To address these limitations, image-based 3D human motion capture using a monocular camera draws an increasing attention recently.

Despite of the remarkable successes achieved on 3D human pose estimation, the single-view based methods suffer from the inherently ambiguity of single-view reconstruction. This ambiguity is often addressed by learning human pose prior from existing MoCap datasets, but the learned prior could produce accurate reconstruction only when the training data is consistent with the motion to be reconstructed. Another line of work aim to leverage the multi-view information to reconstruct dynamic structures, which is often referred to as nonrigid structure from motion (NRSFM). However, the NRSFM methods typically require clean keypoint tracks and sufficiently fast camera motion, both of which are not easy to satisfy in the case of human motion capture from a single camera. 

In this work, we propose a novel system for 3D human motion capture that integrates the state-of-the-art techniques in human pose estimation, NRSFM and autonomous drones: 1) The CNN-based 2D pose estimator trained on large-scale datasets produces reliable 2D pose estimation; 2) The single-view reconstruction with a generic pose prior learned from existing MoCap data further removes outliers in the estimated 2D poses and provides reliable initialization of 3D pose and camera viewpoint estimates; 3) The NRSFM makes use of multi-view information to further refine the reconstructed 3D poses and imposes articulation constraints; 4) The use of a drone for data capture guarantees fast camera motion which is essential for accurate NRSFM. Our system is fully automatic and applicable to any video captured by a commercial drone with active tracking function such as DJI Phantom 4 and Mavic.  
